Computing Galois groups of Ehrhart polynomials in OSCAR

We report on an implementation of Galois groups in the new computer algebra system OSCAR. As an application we compute Galois groups of Ehrhart polynomials of lattice polytope

==> def.tex <==
\usepackage[utf8]{inputenc}
\usepackage[american]{babel}

\usepackage[draft=true]{minted}

\usepackage{amsmath,amssymb,amsthm}
\usepackage{bbm}    

\usepackage{bm}
\usepackage{accents}
\usepackage{mathrsfs}
\usepackage{mathtools}
\usepackage{fixmath}
\usepackage{paralist}
\usepackage{enumerate}
\usepackage{xspace}

\usepackage{stmaryrd}

\usepackage{booktabs}
\usepackage{array}
\usepackage{graphicx}
\usepackage{pgf,tikz}
\usepackage{array}
\usepackage{hyperref}
\usepackage{cleveref}
\usepackage{enumitem}
\usepackage{csquotes}

\usepackage{pgf,tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{patterns}
\usetikzlibrary[positioning]
\usetikzlibrary[fit]
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{calc}

\usepackage{pgfplots}
\pgfplotsset{compat=1.17}

\newcommand\CC{{\mathbb C}}
\newcommand\EE{{\mathbb E}}
\newcommand\NN{{\mathbb N}}
\newcommand\KK{{\mathbb K}}
\newcommand\QQ{{\mathbb Q}}
\newcommand\RR{{\mathbb R}}
\newcommand\Sph{{\mathbb S}}
\newcommand\TT{{\mathbb T}}
\newcommand\ZZ{{\mathbb Z}}

\newcommand\cI{{\mathcal I}}
\newcommand\cP{{\mathcal P}}
\newcommand\cC{{\mathcal C}}
\newcommand\cS{{\mathcal S}}
\newcommand\cF{{\mathcal F}}
\newcommand\cG{{\mathcal G}}
\newcommand\cL{{\mathcal L}}
\newcommand\cM{{\mathcal M}}
\newcommand\cT{{\mathcal T}}
\newcommand\cQ{{\mathcal Q}}
\newcommand\cB{{\mathcal B}}

\newcommand\0{{\mathbf 0}}
\newcommand\1{{\mathbf 1}}

\newcommand\SetOf[2]{\left\{#1 \mid #2\right\}}
\newcommand\smallSetOf[2]{\{#1 \mid #2\}}
\newcommand\bigSetOf[2]{\bigl\{#1 \bigm| #2\bigr\}}
\newcommand\biggSetOf[2]{\biggl\{#1 \biggm| #2\biggr\}}
\newcommand\BiggSetOf[2]{\Biggl\{#1 \Biggm| #2\Biggr\}}
\newcommand\card[1]{\# #1} % cardinality of a set

\DeclareMathOperator\conv{conv}
\DeclareMathOperator\cork{cork}
\DeclareMathOperator\vol{vol}
\DeclareMathOperator\Sym{Sym}
\DeclareMathOperator\Aut{Aut}
\DeclareMathOperator\argmax{arg\,max}
\DeclareMathOperator\Rev{Rev}
\DeclareMathOperator\id{id}
\DeclareMathOperator\SubDiv{\cS}
\DeclareMathOperator\GF{GF}
\DeclareMathOperator\rk{rk}
\DeclareMathOperator\Gr{Gr}
\DeclareMathOperator\TGr{TGr}
\DeclareMathOperator\Dr{Dr}
\DeclareMathOperator\FlDr{FlDr}
\DeclareMathOperator\val{val}

\DeclareMathOperator\Gal{Gal}
\DeclareMathOperator\DP{DP}

\newcommand\SecFan{{\mathfrak S}}
\newcommand\PSubFan{{\mathfrak P}}

\newcommand\dom{\text{dom}}
\newcommand\supp{\text{supp}}
\newcommand\Trop{\RR \cup \{\infty\}}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{conjecture}[theorem]{Conjecture}
\theoremstyle{remark}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{example}[theorem]{Example}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{question}[theorem]{Question}

\newcommand\Julia{\texttt{Julia}\xspace}
\newcommand\polymake{\texttt{polymake}\xspace}
\newcommand\Singular{\texttt{Singular}\xspace}
\newcommand\ANTIC{\texttt{ANTIC}\xspace}
\newcommand\GAP{\texttt{GAP}\xspace}
\newcommand\TOPCOM{\texttt{TOPCOM}\xspace}
\newcommand\mptopcom{\texttt{mptopcom}\xspace}
\newcommand\OSCAR{\texttt{OSCAR}\xspace}
\newcommand\Pari{\texttt{Pari}\xspace}
\newcommand\SageMath{\texttt{SageMath}\xspace}
\newcommand\Magma{\texttt{Magma}\xspace}
\newcommand\Hecke{\texttt{Hecke}\xspace}
\newcommand\latte{\texttt{LattE}\xspace}
\newcommand\normaliz{\texttt{Normaliz}\xspace}
\newcommand\polydb{\texttt{polyDB}\xspace}

\newcommand\arXiv[1]{\texttt{arXiv:#1}}

